Throughput-Optimal Multihop Broadcast on Directed Acyclic Wireless Networks

We study the problem of efficiently broadcasting packets in multi-hop wireless networks. At each time slot the network controller activates a set of non-interfering links and forwards selected copies of packets on each activated link. A packet is considered jointly received only when all nodes in the network have obtained a copy of it. The maximum rate of jointly received packets is referred to as the broadcast capacity of the network. Existing policies achieve the broadcast capacity by balancing traffic over a set of spanning trees, which are difficult to maintain in a large and time-varying wireless network. We propose a new dynamic algorithm that achieves the broadcast capacity when the underlying network topology is a directed acyclic graph (DAG). This algorithm is decentralized, utilizes local queue-length information only and does not require the use of global topological structures such as spanning trees. The principal technical challenge inherent in the problem is the absence of work-conservation principle due to the duplication of packets, which renders traditional queuing modelling inapplicable. We overcome this difficulty by studying relative packet deficits and imposing in-order delivery constraints to every node in the network. Although in-order packet delivery, in general, leads to degraded throughput in graphs with cycles, we show that it is throughput optimal in DAGs and can be exploited to simplify the design and analysis of optimal algorithms. Our characterization leads to a polynomial time algorithm for computing the broadcast capacity of any wireless DAG under the primary interference constraints. Additionally, we propose an extension of our algorithm which can be effectively used for broadcasting in any network with arbitrary topology.

==> extension.tex <==
\section{Extension of the policy $\pi^*$ : Broadcasting in networks containing a single cycle }
In this section we extend the broadcast policy on a DAG to any network containing cycles. We focus predominantly at the case when the network has a single cycle. Although the general ideas presented below can be extended to networks with multiple cycles, the resulting policy becomes complex to implement in a distributed fashion. \\
From the negative result of the lemma \ref{in_order}, we know that any policy ensuring \emph{in-order} packet delivery at every node can not, in general, achieve the broadcast capacity of a network containing cycles. To get around with this difficulty, we introduce the novel idea of broadcasting using multiple \emph{classes} $\mathcal{K}$ of packets. Informally, the idea is as follows : a new incoming packet arriving at the source node is put into some class $k \in \mathcal{K}$. All packets in a class $k\in \mathcal{K}$ are broadcasted while maintaining in-order delivery property within the class $k$, however packets from different classes do not need to respect this constraint. We will show that for a network containing a single cycle, a class size $|\mathcal{K}|=2$ suffices. \\
Before we go to the actual algorithm, we need the following technical lemma from graph theory. 
\begin{lemma}
Consider a directed graph $\mathcal{G}(V,E)$, rooted at $r\in V$. Let $\mathcal{G}$ contain a unique directed cycle $\mathcal{C}$ where $\ldots a-b-c \ldots $ be a part of the cycle ($a,b,c \in V$).  Then, if $\mathcal{G}$ has broadcast capacity of $k$, we can choose a set of $k$ edge-disjoint directed spanning trees (arborescens) in the graph $\mathcal{G}$ in such a way that none of the trees contain the directed edges $(a,b)$ and $(b,c)$ together. 
\end{lemma}

\begin{proof}
Without any loss of generality, we can assume that $k\geq 2$. By Edmonds' theorem, there exist $k$ edge-disjoint spanning tree in the graph $\mathcal{G}$, rooted at $r$. Denote this set of trees $\mathcal{T}$. If none of the trees $t \in \mathcal{T}$ contains the edges $(a,b)$ and $(b,c)$ together, we are done and $\mathcal{T}$ is the desired set of edge-disjoint directed spanning trees. Otherwise, assume that the directed spanning tree $t_1 \in \mathcal{T}$ contains both the edges $(a,b)$ and $(b,c)$. Since the trees in the set $\mathcal{T}$ are edge-disjoint, any other directed spanning tree $t_2 \in \mathcal{T}\setminus \{t_1\}$ does not contain any of the edges $(a,b)$ and $(b,c)$. Finally, we suitably modify the trees $t_1$ and $t_2$ via the following edge-exchange process : since $t_2$ is a directed spanning tree, there must exist an incoming edge $(d,b) \in t_2$ to the node $b$, where $d \neq a$. Also, $d \neq c$ since, $(b,c) \in E$. Now we exchange the edges $(a,b)$ and $(d,b)$ among the trees $t_1$ and $t_2$, i.e., we form $t_1'=t_1 \cup (d,b)\setminus (a,b)$ and $t_2'=t_2 \cup (a,b) \setminus (d,b)$. By noting that the undirected version of the trees $t_1'$ and $t_2'$ does not contain a cycle, it is easy to argue that both $t_1'$ and $t_2'$ are directed spanning trees (arborescens) rooted at $r$ and satisfy the desired property. \\
\textbf{Case 2 : $\mathcal{G}$ contains parallel edges}\\
The basic idea is to imitate the above proof carefully. 
\end{proof}


\section{Extension of the policy $\pi^*$ : Decomposing the Graph into Strongly Connected Components}
We can make use of the DAG policy developed above by first topologically decomposing the graph into strongly connected components and then making use of a two-level routing-scheduling algorithm. Roughly speaking, the overlay DAG topology runs the $\pi^*$ broadcast policy. The 
